Photospheric Radius Expansion and a double-peaked type-I X-ray burst from GRS 1741.9-2853

We present analysis of two type-I X-ray bursts observed by NuSTAR originating from the very faint transient neutron star low-mass X-ray binary GRS 1741.9-2853 during a period of outburst in May 2020. We show that the persistent emission can be modeled as an absorbed, Comptonized blackbody in addition to Fe K$\alpha$ emission which can be attributed to relativistic disk reflection. We measure a persistent bolometric, unabsorbed luminosity of $L_{\mathrm{bol}}=7.03^{+0.04}_{-0.05}\times10^{36}\,\mathrm{erg\,s^{-1}}$, assuming a distance of 7 kpc, corresponding to an Eddington ratio of $4.5\%$. This persistent luminosity combined with light curve analysis leads us to infer that the bursts were the result of pure He burning rather than mixed H/He burning. Time-resolved spectroscopy reveals that the bolometric flux of the first burst exhibits a double-peaked structure, placing the source within a small population of accreting neutron stars which exhibit multiple-peaked type-I X-ray bursts. We find that the second, brighter burst shows evidence for photospheric radius expansion (PRE) and that at its peak, this PRE event had an unabsorbed bolometric flux of $F_{\mathrm{peak}}=2.94^{+0.28}_{-0.26}\times10^{-8}\,\mathrm{erg\,cm^{-2}\,s^{-1}}$. This yields a new distance estimate of $d=9.0\pm0.5$ kpc, assuming that this corresponds to the Eddington limit for pure He burning on the surface of a canonical neutron star. Additionally, we performed a detailed timing analysis which failed to find evidence for quasiperiodic oscillations or burst oscillations, and we place an upper limit of $16\%$ on the rms variability around 589 Hz, the frequency at which oscillations have previously been reported.

==> README <==
README for tablefootnote package, 2014/01/26, v1.1c


TABLE OF CONTENTS
=================

1 Introduction
2 Download
3 Installation
4 Additional Packages
5 Package Compatibility
6 Author/Maintainer
7 Bug Reports
8 Known Problems


1 INTRODUCTION
==============

This LaTeX package provides the command \tablefootnote{...}
to be used in a table or sidewaystable environment.
In those environments \footnote{...} would not work and
would need to be replaced by \footnotemark in the
(sideways)table and \footnotetext{...} after the
(sideways)table environment ended. Additionally the counters
for footnote and (when the hyperref package with option
hyperfootnotes=true is used) Hfootnote would need to be
adjusted manually. Then still the hyperlinks in a
(sideways)table would not work.
When the footnotebackref package is used, \footnotemark and
\footnotetext{...} would need to be redefined.
Just using \tablefootnote{...} in the (sideways)table does
all this automatically. (Compatibility with the
footnotebackref package was achieved without redefining
\footnotemark or \footnotetext.)
Redefining \footnote was not done as to not create conflicts
with other packages.
This material is subject to the LaTeX Project Public License
(LPPL). See http://www.ctan.org/license/lppl1.3
for the details of that license.


2 DOWNLOAD
==========

`tablefootnote' is available on CTAN:
  http://www.ctan.org/pkg/tablefootnote

Running
tex tablefootnote.dtx
generates the files
tablefootnote.ins, tablefootnote.drv, tablefootnote.sty,
and tablefootnote-example.tex.

Also a ZIP file is provided that contains these files,
the manual (tablefootnote.pdf), the compiled example
(tablefootnote-example.pdf), and this README, already
sorted in a TDS tree:
  http://www.ctan.org/install/macros/latex/contrib/
  tablefootnote.tds.zip

3 INSTALLATION
==============

Installation with ZIP file in TDS format
----------------------------------------
The ZIP file `tablefootnote.tds.zip' contains the files
sorted in a TDS tree. Thus you can directly unpack the
ZIP file inside a TDS tree.
(See CTAN:tds.zip for an explanation of TDS.)
Example:
  cd /...somewhere.../texmf
  unzip /...downloadpath.../tablefootnote.tds.zip
Do not forget to refresh the file name database of this
TDS tree.
Example:
  texhash /...somewhere.../texmf

Manual installation
-------------------
a) Download the tablefootnote files from CTAN.
   If necessary, unpack them.
b) Generate the package and driver files:
     tex tablefootnote.dtx
c) Install the file `*.sty' in your TDS tree:
     cp *.sty TDS:tex/latex/tablefootnote/
   Replace `TDS:' by the prefix of your TDS tree
   (texmf directory).
d) Create the documentation (if necessary), e.g.
     pdflatex  tablefootnote.dtx
     makeindex -s gind.ist  tablefootnote.idx
     pdflatex  tablefootnote.dtx
     makeindex -s gind.ist  tablefootnote.idx
     pdflatex  tablefootnote.dtx
e) Update the databases if necessary, e.g. for teTeX:
     mktexlsr .../texmf
f) Create the tablefootnote-example.pdf (if necessary), e.g.
     pdflatex tablefootnote-example.tex
     pdflatex tablefootnote-example.tex
     pdflatex tablefootnote-example.tex
g) Copy the documentation files to
   "TDS:doc/latex/tablefootnote/":
   README, tablefootnote.pdf, tablefootnote-example.tex,
   tablefootnote-example.pdf.


4 ADDITIONAL PACKAGES
=====================

tablefootnote loads other packages:
* letltxmacro, http://www.ctan.org/pkg/letltxmacro
* ltxcmds, http://www.ctan.org/pkg/ltxcmds
When the etoolbox package is available, it is used:
* etoolbox, http://www.ctan.org/pkg/etoolbox
(All packages possibly load further packages.
See the result of the \listfiles command in the log-file
of the example.)


5 PACKAGE COMPATIBILITY
=======================

- Using the hyperref-option pdfview=FitH or FitBH makes the
    hyperlinks of footnotes in sidewaystables to not lead
    to the footnotes, due to a bug in pdfTeX,
    computing wrong anchor coordinates (Heiko Oberdiek,
    29. October 2011). The printed version is OK.
- Footnotes in sidewaystables are printed one below the
    other, even if the footmisc package with option "para"
    is used.
- When LuaTeX is used to compile a document with
    rotated content, the hyperreferences therein are
    misplaced (regardless of loaded tablefootnote-package
    or footnotes at all - all hyperreferences in
    rotated content are misplaced). Using pdflatex does not
    result in any problem here.


6 AUTHOR/MAINTAINER
=====================

* H.-Martin Münch


7 BUG REPORTS
==============

A bug report should contain:
* Comprehensive problem description. This includes error or
  warning messages.
* \errorcontextlines=\maxdimen can be added in the
  TeX code to get more information in TeX error messages.
* Minimal test file that shows the problem, but does not
  contain any unnecessary packages and code.
* Used drivers/programs.
* Version information about used packages and programs.
* If you are using LaTeX, then add "\listfiles". Then
  a list of version information is printed at the end
  of the LaTeX run.
* Please no other files than the minimal test file.
  The other files .log, .dvi, .ps, .pdf are seldom
  necessary, so send them only on request.
* Please .zip or .tar.gz your file(s) before sending them!

Bug address
-----------
Bug reports can be send to the maintainer:
  H.-Martin Münch
  <Martin [dot] Muench [at] Uni-Bonn [dot] de>


8 KNOWN PROBLEMS
=================

- Using the hyperref-option "pdfview=FitH" or "pdfview=FitBH"
    makes the hyperlinks of footnotes in sidewaystables
    to not lead to the footnotes, due to a bug in pdfTeX,
    computing wrong anchor coordinates (Heiko Oberdiek,
    2011/10/29). The printed version is OK.
- Footnotes in sidewaystables are printed one below the other,
    even if the footmisc package with option para is used.
- When a table with (table)footnotes floates to another place,
    its footnotenumbers are not automatically adapted.
- When LuaTeX is used to compile a document with
    rotated content, the hyperreferences therein are
    misplaced (regardless of loaded tablefootnote-package
    or footnotes at all - all hyperreferences in
    rotated content are misplaced). 
    Using pdflatex does not result in any problem here.
    Problem found by Arno Trautmann, 2011/11/15.

Ideas for solutions are welcome!
